WAFFLE: Watermarking in Federated Learning

Federated learning is a distributed learning technique where machine learning models are trained on client devices in which the local training data resides. The training is coordinated via a central server which is, typically, controlled by the intended owner of the resulting model. By avoiding the need to transport the training data to the central server, federated learning improves privacy and efficiency. But it raises the risk of model theft by clients because the resulting model is available on every client device. Even if the application software used for local training may attempt to prevent direct access to the model, a malicious client may bypass any such restrictions by reverse engineering the application software. Watermarking is a well-known deterrence method against model theft by providing the means for model owners to demonstrate ownership of their models. Several recent deep neural network (DNN) watermarking techniques use backdooring: training the models with additional mislabeled data. Backdooring requires full access to the training data and control of the training process. This is feasible when a single party trains the model in a centralized manner, but not in a federated learning setting where the training process and training data are distributed among several client devices. In this paper, we present WAFFLE, the first approach to watermark DNN models trained using federated learning. It introduces a retraining step at the server after each aggregation of local models into the global model. We show that WAFFLE efficiently embeds a resilient watermark into models incurring only negligible degradation in test accuracy (-0.17%), and does not require access to training data. We also introduce a novel technique to generate the backdoor used as a watermark. It outperforms prior techniques, imposing no communication, and low computational (+3.2%) overhead.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}

\subsection{Discussion and Takeways}\label{ssec:discussion}
 
In contrast to existing Pre- and Post-embedding techniques, \ourmethod\ meets \ref{req:w_ownership} enabling to reliably demonstrate ownership of $w_{G}$ at any aggregation round. 
\ourmethod with \ourpattern meets every requirement set in Section~\ref{ssec:requirements} as summarized in Table~\ref{tb:wmsetssummary}. \ourpattern is the most suitable watermark set for watermarking federated learning models since it provides the best trade-off between performance and robustness across the different datasets tested.


\begin{table}[!ht]
\caption{Ranking (1-4) for meeting the requirements set in Section~\ref{ssec:requirements} for different watermark sets. MNIST (left) and CIFAR10 (right) tasks.}\label{tb:wmsetssummary}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular} {| p{\dimexpr 0.40\linewidth-2\tabcolsep}
                       | p{\dimexpr 0.22\linewidth-2\tabcolsep}
                       | p{\dimexpr 0.20\linewidth-2\tabcolsep}
                       | p{\dimexpr 0.19\linewidth-2\tabcolsep}
                       |p{\dimexpr 0.19\linewidth-2\tabcolsep}|}
\hline 
\textbf{MNIST/CIFAR10}&  \hfil \ourpattern & \hfil Embedded C. & \hfil unRelate & \hfil unStruct \\ \hline
~\ref{req:w_ownership} Demonstration of ownership & \hfil 1/1 & \hfil 2/3 & \hfil 3/2 & \hfil 3/3\\ \hline
~\ref{req:w_robustness} Robustness (Fine-tuning) & \hfil 2/1 & \hfil 4/4 & \hfil 3/3 & \hfil 1/2\\ \hline
~\ref{req:w_robustness} Robustness (Pruning) & \hfil 2/1 & \hfil 4/4 & \hfil 3/2 & \hfil 1/3\\ \hline
~\ref{req:w_robustness} Robustness (Neural Cleanse) & \hfil 3/3 & \hfil 4/2 & \hfil 2/1 & \hfil 1/4\\ \hline
~\ref{req:w_data_independence} Data Independence & \hfil Yes/Yes & \hfil No/No & \hfil Yes/Yes & \hfil Yes/Yes\\ \hline
~\ref{req:p_utility} Model utility & \hfil 2/3 & \hfil 1/4 & \hfil 3/1 & \hfil 4/2\\ \hline
~\ref{req:p_communication} Comm. overhead & \hfil 2/3 & \hfil 1/4 &\hfil  3/1 & \hfil 4/2\\ \hline
~\ref{req:p_computation} Comput. overhead & \hfil 3/2 & \hfil 2/3 &\hfil  4/4 & \hfil 1/1\\ \hline
\end{tabular}}
\end{table}


\ourmethod is also resilient to all watermark removal attacks if less 
than 40\% clients are malicious, as summarized in Table~\ref{tb:overallresilience}. While Neural Cleanse requires only 10\% malicious clients to be successful against the CIFAR10 model, adversaries would have to share their datasets and collaborate with each other to recover the triggers.
The collaboration between adversaries in a distributed attack is different from the sybil attack in our case. Creating multiple identities does not improve removal and evasion attacks since the performance of these attacks is directly related to the amount and the diversity of data held by the adversary. 
Collaboration is impractical since adversaries need to reveal their highly-sensitive dataset to other untrustworthy parties. 
On the other hand, if an adversary holds more than 10\% of the whole training data, it could successfully remove watermarks from $w_{adv}$ without decreasing the model performance. This scenario is not realistic in a federated learning setup because a client having such an amount of data could directly train its own model locally without taking part in federated learning to eventually steal the model. We conclude that under reasonable assumptions, \ourmethod is resilient to distributed attacks of several malicious federated learning clients.

\begin{table}[!ht]
\caption{Minimum ratio of malicious clients required to evade \ourmethod.}\label{tb:overallresilience}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{c|c|c}
 \hline 
 \textbf{Attack type}  & \textbf{MNIST} & \textbf{CIFAR10} \\ 
 \hline 
 Fine-tuning~\cite{yosinski2014transferable} & 50\% & 50\% \\ 
 \hline 
 Pruning~\cite{han2015learning} & 40\% & 40\%  \\ 
 \hline 
 Neural Cleanse, patching-via-unlearning~\cite{wang2019neural} & 40\% & 10\% \\ 
 \hline
Evasion of verification with OOD detection~\cite{li2019prove} & - & 50\% \\ 
 \hline 
 \end{tabular}}  
 \end{table}
 
In addition to methods to recover and remove watermarks, an adversary can also attack the verification mechanisms~\cite{adi2018turning,szyller2019dawn} used to demonstrate model ownership. Even though verification in not in the scope of our paper we discuss these attacks.
An adversary may try to \textit{evade verification} by detecting queries for watermark samples as out-of-distribution (OOD) samples. We implemented and tested this attack using the threshold-based detector model introduced in~\cite{li2019prove}. We show that \ourmethod watermark verification could be evaded if the adversary has high quality IID data. However, \ourmethod is resilient to evasion in a non-IID setting (details in Appendix~\ref{app:evasion}). 

An adversary can also try to cast model ownership into doubt by embedding its own watermark into the model: \textit{ownership piracy}.
This issue can be addressed by registering any watermark into a time-stamped bulletin (e.g., blockchain) for it to be valid~\cite{adi2018turning,szyller2019dawn}. We can enforce our watermark to be registered together with some private artifacts of the model before federated learning starts  as a proof of authenticity. 
Such a private artifact can be the architecture of the model (number of layers, number of neurons, type of activation functions, etc.) since all these parameters are unknown to any federated learning client before they receive the initial model. 

Finally, a model stealing attack can be performed against $w_{adv}$ by the adversary itself to create a surrogate model without watermark~\cite{shafieinejad2019robustness,szyller2019dawn}. Model stealing typically requires a large amount of data (more than specified by our adversary model) and it causes accuracy drops larger than 5\% ~\cite{atli2019extraction}. Thus, we consider these attacks as impractical in our adversary model.

  
While we focused on a single owner $O$. in this paper, \ourmethod can also be used where \client s would all be owners of the trained model. In this case, the aggregator can generate and distribute different subsets of the watermark set to each client for individual demonstration of ownership. There are challenges to be addressed in the case of collective ownership since the size of the watermark set increases linearly with the number of owners and there might be a decrease in utility. We consider extending \ourmethod to this case as future work. \newtext{We will also explore how malicious clients can try to recover and degrade watermarks \textit{during} the federated learning training and to detect the presence of these adversaries.}   

%\section{Acknowledgments}\label{sec:acknowledgments}
%This work was supported in by the Intel (ICRI-CARS). 
%We thank the computational resources provided by the Aalto Science-IT project.

